GraphZeppelin: Storage-Friendly Sketching for Connected Components on Dynamic Graph Streams

Finding the connected components of a graph is a fundamental problem with uses throughout computer science and engineering. The task of computing connected components becomes more difficult when graphs are very large, or when they are dynamic, meaning the edge set changes over time subject to a stream of edge insertions and deletions. A natural approach to computing the connected components on a large, dynamic graph stream is to buy enough RAM to store the entire graph. However, the requirement that the graph fit in RAM is prohibitive for very large graphs. Thus, there is an unmet need for systems that can process dense dynamic graphs, especially when those graphs are larger than available RAM. We present a new high-performance streaming graph-processing system for computing the connected components of a graph. This system, which we call GraphZeppelin, uses new linear sketching data structures (CubeSketches) to solve the streaming connected components problem and as a result requires space asymptotically smaller than the space required for a lossless representation of the graph. GraphZeppelin is optimized for massive dense graphs: GraphZeppelin can process millions of edge updates (both insertions and deletions) per second, even when the underlying graph is far too large to fit in available RAM. As a result GraphZeppelin vastly increases the scale of graphs that can be processed.

==> core_system.tex <==
%!TEX root =  main.tex




==> distributed.tex <==

%!TEX root =  main.tex



==> external_memory_system.tex <==
%!TEX root =  main.tex

We use a write-optimized buffer tree as an intermediary in stream ingestion. We think of the buffer tree as a black box that consumes stream updates and lazily produces buffers of updates destined for particular node sketches. When we issue a connectivity query, we force the tree to flush and produce all of the update buffers it can.

When we receive a stream update $((u,v),\Delta)$, we write two copies of it into the top-level buffer $(u,(v,\Delta))$, $(v,(u,\Delta))$, one for each endpoint of the update. We will refer to the first argument of these written copies as the \say{destination} node. For example, $u$ is the destination node in the update structured $(u,(v,\Delta))$. We index the buffer tree by destination node so that leaf buffers only contain updates with the same destination.

If the root buffer becomes too full, we first run a "heavy-hitters" algorithm indexed on destination node. If there are any nodes that have many updates, we push them to the appropriate node sketch for processing and re-format the buffer without these updates. If the buffer is still too full, we flush it to its children buffers. Non-root internal buffers are flushed at a similar load threshold. Leaf buffers are flushed by pushing the contents (stream updates with the same destination node) as a buffered update.

If a connectivity query made, we force a flush of every buffer, from the root down.

Note the buffer tree specification thus far makes no reference to the underlying storage for the updates or the buffer. In practice, since we may have many levels in the tree and many stream updates, we store the majority of the tree on disk. We keep only the root buffer, metadata for other buffers, and synchronization tools persistently in memory. As an optimization, we pre-declare enough disk space for the entire tree structure and write directly to locations in the tree file when a flush necessitates it.

% TODO Evan: Add more notes about disk/implementation


==> externalmemory.tex <==
%!TEX root =  main.tex

\section{External memory graph algorithms}

\begin{definition}An external graph $G = (V,E)$ is a graph stored on disk, typically in adjacency list format. Scanning in the adjacency list of a node $n$ requires $|N(n)|/B$ I/Os where $N(n)$ is the set of neighbors of $n$.
\end{definition}

\begin{definition}
An external graph $G = (V,E)$ is sparse if $|V| > |E|/B$.
\end{definition}


\begin{theorem}External Memory CC can be solved using $O(sort(|E|) * max\{1, \log \log (|V|BD/ |E|\})$
\end{theorem}
This theorem is given by Irit Katriel and Ulrich Meyer in ``Elementary Graph Algorithms in External Memory.''

The simple version of this algorithm works through a number of rounds where nodes are combined into super-nodes if they are members of the same \textbf{pseudo-tree}. These pseudo-trees are constructed by having each node create an edge with it's smallest neighbor. We then combine all the nodes in the same pseudo-tree and remove all edges except those between the new super-nodes. This process repeats iteratively until the graph is small enough for external memory BFS to be effective.

BFS is not effective before running these iterations because the graph may be quite dense. In addition to shrinking the number of nodes these iterations dramatically reduce their degree. Therefore, the iterations run until the graph is sparse.


sorting two copies of the edges, one by source node and the other by target node, and


==> figures/supernode_example.tex <==
\begin{figure}[!t]
    \centering
    \[ \begin{blockarray}{r*{6}{ >{}c}}
& (1,2) & (1,3) & (1,4) & (2,3) & (2,4) & (3,4) \\ \\
\begin{block}{ >{\scriptstyle}r!{\,}(cccccc)}
x_{1} & 0 & 1 & 1 & 0 & 0 & 0 \\
x_{2} & 0 & 0 & 0 & 1 & 0 & 0 \\
x_{3} & 0 & -1 & 0 & -1 & 0 & 1 \\
x_{4} & 0 & 0 & -1 & 0 & 0 & -1 \\
x_{1}+x_{4} & 0 & 1 & 0 & 0 & 0 & -1 \\
\end{block}
\end{blockarray} \]%
\usetikzlibrary{positioning,calc,fit,shapes}
%\tikzset{main node/.style=,}
\begin{tikzpicture}  
  [auto,
 block/.style ={circle,fill=blue!20,draw,minimum size=.5cm,inner sep=0pt},
] % here, node/.style is the style pre-defined, that will be the default layout of all the nodes. You can also create different forms for different nodes.  
    
   \node[block] (b) at (0,0) {$2$}; 
   \node[block] (c) [right =of b] {$3$};  
   \node[block] (a) [below =of b] {$1$};  
   \node[block] (d) [below =of c] {$4$};  
   \draw (a) -- (c);  
   \draw (a) -- (d);  
   \draw (b) -- (c);
   \draw (c) -- (d); 
   \node[rectangle,draw=black, fit=(a) (d)](FIt1) {};
 
   
  
\end{tikzpicture}  
    \caption{\sysname Characteristic vectors of the graph. }
    \label{fig:supernode_example_table}
\end{figure}





==> improvement.tex <==
%!TEX root =  main.tex

\section{Shortcomings of the Basic Algorithm (will disappear soon)}
\label{sec:improvement}
\david{TODO: I feel like there's a ordering issue here.  We have to describe implementation details of a sketching algorithm we haven't described here, then 
- explanation of sketch size: mention that sketches require $\O(log^2(\nodesize^2))$ integers which can take on values up to $\nodesize^2c$ for constant $c$ and even for $c = 2$ this requires the use of 128 bit ints.
- redo the second paragraph's math: use our estimate of Aspen's memory use.  make the point that we are targeting cases where our data structure is smaller than in-memory solutions like aspen, and at those sizes our data structure is way too slow to use.
The last pieces of this section feel more like parts of an intro.
we need to redo kenny's sketch update speed experiment
add a section here about how this basic algorithm has to do each update individually, limiting the benefits of parallelism and making disk usage horrible.  how can we clearly argue that it impedes parallelism?  just through experiment?  can we set up such an experiment easily?}
\algname requires sketching vectors of length $V^2$, and as a result the 1-sparse recovery procedure in $\ell_0$ sampling requires storing 3 128-bit integers.  Each per-node sketch requires $\log^3(V^2) = 8 \log^3(V)$ of these sparse recovery data structures so the total data structure size is $384n \log^3(V)$.  For a graph with a million nodes, this data structure is about 3 TB in size.  Each update requires $\log^3(V)$ modular exponentiation operations which each in turn require $O(\log(V))$ modulus and multiplication operations.  This high update cost is further exacerbated by the computational overhead required for performing arithmetic operations on 128-bit integers on current-generation hardware.  For these reasons, a straightforward single-threaded implementation of Ahn \etal's algorithm using this $\ell_0$ sampling procedure is quite slow: in Fig. x we show the update rate of this algorithm for graphs of various sizes.  The sketch data structure can process approximately 20 edge updates per second on a graph with a million nodes. \david{add experimental data here.}

%\input{figures/l0speedup}

The goal of \algname is to use smaller space than would be required to store the entire graph in memory explicitly.  While the sketch data structure is asymptotically smaller than an adjacency list (for dense graphs) or an adjacency matrix, in practice it is only smaller than the Boost adjacency matrix representation for graphs of about 2 million nodes (for dense graphs, any adjacency list representation is much larger than that of an adjacency matrix).  On a dense graph, say with $V^2/4$ = 1 trillion edges, 0.08 seconds/edge * 1 trillion = 2.5 millennia.  This interminable runtime only gets worse for graphs that are larger or have more edges, so with current hardware this straightforward implementation of the sketching algorithm is only space-efficient for graphs which are infeasible for computation.

To overcome these shortcomings, in this work we introduce a series of optimizations which make the \sysname core algorithm not only practical but far better than existing techniques for computing connectivity queries on live turnstile graph streams.  First we present an improvement on the $\ell_0$-sketching procedure for this specific application which decreases the update time by a $\log(V)$ factor (and reduce the number of hash function calls, a limiting factor for runtime in practice, by an additional $\log(V)$ factor) and reduces the space by a large constant factor (around 20x).  These improvements are stated and proved in Section~\ref{sec:theory}.  As a result of these optimizations, we observe a runtime improvement of 2000x over the naive algorithm and we further find that the algorithm outperforms standard in-memory connected components algorithms on workloads which it can process in a few hours.  We further improve its performance with multithreading, external memory buffering, and a distributed implementation for the Spark framework, and further reduce the space requirements by establishing experimentally that the failure probability in practice is much lower than the theoretical upper bound.  Experiments establishing the value of each of these optimization techniques are presented in Section~\ref{sec:experiments}.


==> titleauth_bad.tex <==
%!TEX root =  main.tex

\title{\sysname: Storage-Friendly 
% Linear Kvetching
Sketching
for Connected Components on Dynamic Graph Streams.}

% \sysname: using storage to extend the reach of sketches in dynamic streaming graphs

% \sysname: Streaming Connected Components on Large, Dynamic Graphs using Linear Sketching

\author{David Tench}
\affiliation{%
  \institution{Rutgers University}
  %\country{USA}
}
\email{dtench@pm.me}

\iffalse
\author{Evan West}
\affiliation{%
  \institution{Stony Brook University}
  
  %\country{USA}
}

\author{Victor Zhang}
\affiliation{%
  \institution{Rutgers University}
  \email{victor@vczhang.com}
  %\country{USA}
}

\author{Michael A. Bender}
\affiliation{%
  \institution{Stony Brook University}
  %\country{USA}
    \email{bender@cs.stonybrook.edu}
}

\author{Abiyaz Chowdhury}
\affiliation{%
  \institution{Stony Brook University}
  \email{abchowdhury@cs.stonybrook.edu}
  %\country{USA}
}

\author{J. Ahmed Dellas}
\affiliation{%
  \institution{Rutgers University}
  \email{jad525@scarletmail.rutgers.edu}
  %\country{USA}
}

\author{Martin Farach-Colton}
\affiliation{%
  \institution{Rutgers University}
  \email{martin@farach-colton.com}
  %\country{USA}
}

\author{Tyler Seip}
\affiliation{
  \institution{MongoDB}
}

\author{Kenny Zhang}
\affiliation{%
  \institution{Stony Brook University}
  \email{kzzhang@cs.stonybrook.edu}
  %\country{USA}
}
\fi
  
\renewcommand{\shortauthors}{Tench, West, and Zhang et al.}

